Rethinking Incentives in Recommender Systems: Are Monotone Rewards Always Beneficial?

The past decade has witnessed the flourishing of a new profession as media content creators, who rely on revenue streams from online content recommendation platforms. The reward mechanism employed by these platforms creates a competitive environment among creators which affect their production choices and, consequently, content distribution and system welfare. It is thus crucial to design the platform's reward mechanism in order to steer the creators' competition towards a desirable welfare outcome in the long run. This work makes two major contributions in this regard: first, we uncover a fundamental limit about a class of widely adopted mechanisms, coined Merit-based Monotone Mechanisms, by showing that they inevitably lead to a constant fraction loss of the optimal welfare. To circumvent this limitation, we introduce Backward Rewarding Mechanisms (BRMs) and show that the competition game resultant from BRMs possesses a potential game structure. BRMs thus naturally induce strategic creators' collective behaviors towards optimizing the potential function, which can be designed to match any given welfare metric. In addition, the BRM class can be parameterized to allow the platform to directly optimize welfare within the feasible mechanism space even when the welfare metric is not explicitly defined.

==> theory.tex <==
 \section{The Price of Anarchy Analysis} 

We analyze the social welfare of any top-$K$ RS under any possible CCE; or more specifically, \emph{how bad can the welfare possibly be due to the competition among self-interested content creators} -- compared to the \emph{idealized} non-strategic situation in which the platform can ``dictate'' all creators' content choices and thus globally optimize the welfare function \eqref{eq:welfare_original}. This can be captured by the celebrated concept of the Price of Anarchy (PoA) \citep{koutsoupias1999worst}. As its name indicates, PoA captures the welfare inefficacy due to players' selfish behavior. Our main result in this section is a comprehensive characterization of the PoA of \game{}s. %Intuitively, PoA is   the ratio between the maximum possible   welfare  and the worst-case   welfare induced by any equilibrium,   formally defined as follows:
\begin{definition}[PoA under CCE]
Define the price of anarchy of a game $\G$ as 
\begin{equation}\label{eq:poa_def}
        PoA(\G)=\frac{\max_{\s\in\S}W(\s)}{\min_{\al\in CCE(\G)}\EE_{\s\sim \al}[W(\s)]},
\end{equation}
where CCE$(\G)$ is the set of CCEs of $\G$.  
\end{definition}

By definition, PoA$(\G)\geq 1$ always holds and larger values indicate worse welfare. Our choice of the CCE concept leads to the strongest possible welfare guarantee in the sense that any upper bound of PoA under CCE also trivially holds for the PoA under refined solution concepts such as correlated equilibrium (CE), PNE or mixed NE (if they exist), since these are all CCEs as well. Unless otherwise emphasized, any PoA in this paper refers to the PoA under CCE. 

% because it is a broad generalization of NE which is easy to compute and learn: it is known that if each player adopts a no-regret algorithm to update their strategy, the averaged sequence of actions converges to an approximated CCE. Since the set of CCE includes all correlated equilibria (CE), mixed Nash equilibria (MNE), and NE, our main result regarding the welfare guarantee automatically applies to all the solution concepts mentioned above, if they exist at all \footnote{The concept of PoA typically refers to the PoA of NE. However, for those reasons mentioned above, we consider the PoA of CCE throughout this work.}. 

% \hf{I think  Theorem 1 and Theorem 2 should both be moved here.  When writing the paper, we should try to present our main result as early as possible and use the minimum possible background knowledge possible. Any technical issues relevant to the proof of the theorem should come afterwards, NOT before it. }

% \hf{Maybe the following is a better flow for arranging contents of this section. 

% 1. Say "The main result of this paper is the following tight characterization about the price of anarchy of the engagement game." then state your theorem. 

% 2. Explain the various important implications of your two theorems, show how amazing your results are. (Only when the audience is convinced by how amazing your results are, they are willing to spend time reading your proofs. )

% 3. Explain the high-level ideas of your proof, and highlight the challenges of the proofs. (At this point, you are trying to convince the audience that your results are not only theoretically insightful but are highly non-trivial to prove). 

% 4. Present the detailed proofs of the two theorems in two separate subsections. This is the place to put your technical definitions. This sections are written for those who truly want to understand details of your proof. This part can be put into the appendix if we need space, but for EC we should put at least the proof of Theorem 1 in the main body I think.  (This part is to convince the readers from our own field that   our results are highly non-trivial.)} 

\subsection{Matching PoA Upper and Lower Bounds}\label{sec:main_result}

Our main theoretical findings are an upper and lower bound for the PoA, which match with each other and thus demonstrates the tightness of our analysis. We first present the upper bound as follows.

\begin{theorem}\label{thm:PoA}
% For any $\beta\geq0, K\geq 1$, the PoA of any \game{} instance $\G(\{\S_i\}_{i=1}^n, \X, \sigma, \beta, K)$ satisfies
The PoA of any \game{} instance $\G$ with parameter  $\beta\geq0$ and $K\geq 1$  satisfies % \hf{Do we need any assumption on the scoring function $\sigma$?}
\begin{equation}\label{eq:PoA_main}
    PoA(\G) < 1+ \frac{1}{c(\beta,K)},
\end{equation}
where $c(\beta, K)$ is defined as

\begin{align}\label{eq:cbetaK_def}
c(\beta, K)= \frac{(b+1)\log(b+K)}{(b+K)(\log(b+K)-\log K)}, b=e^{\frac{1}{\beta}}-1.
\end{align}    

\end{theorem}
The proof of Theorem \ref{thm:PoA} is intricate and thus the detailed arguments are relegated to Appendix \ref{app:poa_proof}. The primary challenge in the proof is to analyze various smoothness properties of the welfare and players' utility functions, especially how the welfare function changes after excluding any player $i$'s participation. In Section \ref{subsec:proof-sketch}, we highlight some of the noteworthy properties of the welfare function, including its submodularity, which we develop en route to proving Theorem \ref{thm:PoA} but is also of independent merit towards understanding the \game{}.   
 
The format of $c(\beta, K)$ may not be intuitive enough for the readers to appreciate the derived PoA upper bound. We thus provide the following observations, which reveal various properties of $c(\beta, K)$ aiding the interpretation of \eqref{eq:PoA_main}:
%\begin{observation}\label{coro:cbetak}
%We make the following observations on the constant $c(\beta, K)$:
\begin{enumerate}
    \item For any $\beta>0$ and $K\geq 1$, we have $c(\beta, K)\geq 1$ and thus PoA$(\G) < 2$ always holds.

    \item $c(\beta, K)=1$ if and only if $K=1$ or $\beta \rightarrow 0$.
    
    \item Fix any $\beta>0$, $c(\beta, K)$  monotonically increases in $K$; similarly, fix any $K\geq 1$, $c(\beta, K)$ monotonically increases in $\beta$.
    
    \item For sufficiently large $\beta$ and $K$, $c(\beta, K) \approx (1+\beta)\log K$ asymptotically, and therefore 
    \begin{equation}\label{eq:PoA_upper}
        PoA(\G) < 1+\frac{1}{(1+\beta)\log K}.
    \end{equation}
\end{enumerate}
%\end{observation}

Based on these observations, Theorem \ref{thm:PoA} has multiple interesting and immediate implications. First, the welfare loss under any CCE is at most half in any situation, as the PoA is always upper bounded by 2. The second and third facts above show that such worst-case PoA occurs and only occurs when users' choices are made in a ``hard" manner: either the RS dictates the user's choice by setting $K=1$ or the randomness in users' choices is extremely low (i.e., $\beta \rightarrow 0$). Note that in the latter case, the user will only consume the most relevant content (i.e., the top-ranked content) due to small decision randomness.   

Second, the welfare guarantee improves as either $K$ increases (i.e., more items are recommended) or $\beta$ increases (i.e., users' choices have more randomness). Welfare improvement in the latter situation is intuitive because when supplied with multiple items, the user can pick the content with large $\varepsilon_i$ (i.e., the reward component that is not predictable by the RS) to gain utility. These together reveal an interesting operational insight that when the RS cannot perfectly predict user utility (i.e., $\beta > 0$), providing more items can help improve social welfare. This justifies top-$K$ recommendation and the necessity of diversity in recommendation \citep{hurley2011novelty}.   

%Finally, Theorem \ref{thm:PoA} also quantitatively provides the precise order, to which the increase of $K$ or $\beta$ can help to increase the welfare guarantee. Concretely,  the asymptotic relationship between PoA and $(\beta,K)$ is given by \eqref{eq:PoA_upper}.  

Our following second main result shows that this PoA upper bound is tight, up to negligible constants. 

% Now we present a lower bound result to demonstrate the tightness of the PoA bound in Theorem \ref{thm:PoA}. Rigorously, we establish an asymptotic matching lower bound for PoA for sufficiently large $n$ in the following Theorem: 

\begin{theorem}\label{thm:PoA_lowerbound}
  Given any $0\leq\beta\leq 1 $, $n > 2$ and any $1\leq K\leq \min\{n-1, e^{\frac{1}{5\beta}}\}$, there exists a \game{} instance $\G(\{\S_i\}_{i=1}^n, \X, \sigma, \beta, K)$ such that
    \begin{equation}
        PoA(\G)> \frac{n-1}{n}+\frac{1}{1+5\beta\log K}.
    \end{equation}
\end{theorem}
This theorem also implies that the argument we employed for Theorem \ref{thm:PoA}, which is based on the \emph{smoothness} proof developed by \citet{roughgarden2015intrinsic}, yields a tight PoA bound for our proposed game. The tightness of the smoothness argument is itself an intriguing research question. Only three classes of games are known to enjoy a tight PoA bound derived from the smoothness argument: congestion games with affine cost \citep{christodoulou2005price}, second price auctions \citep{christodoulou2008bayesian}, and the valid utility game \citep{vetta2002nash},  which are all fundamental classes of games. Theorem \ref{thm:PoA_lowerbound} suggests that our \game{} subscribes to this list. The proof of Theorem \ref{thm:PoA_lowerbound} is to explicitly construct a game instance which provably yields the stated PoA lower bound (see Appendix \ref{app:poa_lower_proof}). 


% In really, it is unlikely to encounter deterministic user behavior or encounter an RS that dictates what content users should consume. Therefore, Theorem \ref{thm:PoA} suggests that we should expect a much better   welfare guarantee than a factor of $2$ even under the basic top-$K$ RS. 


 

% that the welfare guarantee keeps improving when $K$ or the variance level of user decision noise $\beta$ become larger. However, in the worse case, the user welfare at the CCE is at least half of the optimal welfare. 



\subsection{Implications of the PoA Bounds} \label{sec:imp_poa}

% \fan{discuss how our result connects to \cite{ben2019recommendation}, \cite{shen2016hotelling} } 
We have discussed some direct implications of  Theorem \ref{thm:PoA}. Now we develop new results which are either derived from or can be compared to Theorem \ref{thm:PoA} and \ref{thm:PoA_lowerbound}. They will reveal additional insights from our main theoretical results.

\vspace{2mm}
\noindent 
\textbf{Welfare implications to \emph{learning} content creators. }  
The PoA bounds presented in Theorem \ref{thm:PoA} and \ref{thm:PoA_lowerbound} are based on the assumption that creators are aware of the game parameters and play some CCEs of the game. While CCE is a reasonable equilibrium concept, one potential critique is that to find the CCE, it is assumed that each creator has knowledge about the system parameters (e.g., all other creators' strategies and the $\sigma$ function), which can be unrealistic. Fortunately, in real-world scenarios where creators utilize no-regret algorithms to play a repeated \game{} with bandit feedback, we can still establish a slightly worse PoA upper bound leveraging the fact that the average strategy history of no-regret players converges to a CCE, as shown in the following Corollary \ref{coro:noregret_CCE}.

\begin{corollary}\label{coro:noregret_CCE}[\textbf{Dynamic Version of Theorem \ref{thm:PoA}}]
Suppose each player in a repeated \game{}  $\G(\{\S_i\}_{i=1}^n, \X, \sigma, \beta, K)$ independently executes some no-regret learning algorithm, with worst   regret $R(T) = \max_i R_i(T)$ as defined in \eqref{def:regret}. Then we have
% \begin{small}
\begin{equation}\label{eq:PoA_noregret}
\frac{\max_{\s\in\S}W(\s)}{\frac{1}{T}\sum_{t=1}^T \EE_{\s \sim \al^t}[W(\s)]}
< 1+\Big(1+\frac{n}{\beta\log K}\cdot \frac{R(T)}{T}\Big)\cdot \frac{1}{c(\beta,K)}, 
\end{equation}
% \end{small}
where $\al^t$ denotes the joint-strategy distribution at step $t$ and $c(\beta,K)$ is the constant defined in  \eqref{eq:cbetaK_def}.
\end{corollary}
In other words, the average welfare across all rounds $\frac{1}{T}\sum_{t=1}^T \EE_{\s \sim \al^t}[W(\s)]$ is close to the maximum possible welfare $\max_{\s\in\S}W(\s)$, up to a constant factor. The quantity in the LHS of \eqref{eq:PoA_noregret} is also known as the ``price of total anarchy"  \cite{blum2008regret}. It is a substitute for PoA when we want to characterize the welfare of an outcome from repeated play which does not necessarily fall into any equilibrium concept. The proof of Corollary \ref{coro:noregret_CCE} is presented in Appendix \ref{app:poa_proof_regret}. Because $R(T)/T \rightarrow 0$ as $T \rightarrow \infty$ for any no-regret algorithm (most no-regret algorithms have $R(T) = O(\sqrt{T})$), the RHS of \eqref{eq:PoA_noregret} is still strictly less than 2 for any fixed constants $(n,\beta,K)$. 
% Similarly, we can see that the welfare guarantee improves as $\beta$ or $K$ increase and decreases as the number of players $n$ increases.

Theorem \ref{thm:PoA} relies on two crucial platform features: 1. the player's utility in \eqref{eq:player_utility_original} is defined as the total user engagement that accounts for the user utility $\sigma(\s_i, \x_j) + \varepsilon_j$, as opposed to just ``user exposure'' (i.e., the expected total number of matches); 2. the platform uses the top-$K$ recommendation policy. Next, we illustrate the insights revealed from Theorem \ref{thm:PoA} with respect to these two key features. 


\vspace{2mm}
\noindent
\textbf{The importance of rewarding user engagement rather than solely exposure. } 
 A key reason for the nice PoA guarantee in our \game{} is each player $i$'s  utility is chosen as the user engagement $\sum_j \EE[\sigma(\s_i, \x_j)+\varepsilon_i|\x_j \shortrightarrow \s_i]   \Pr(\x_j \shortrightarrow \s_i)$  in \eqref{eq:player_utility_original}, while not the following user exposure metric: 
 \begin{equation}\label{eq:player_utility_new}
     \text{User exposure for player }i: \quad  \sum_{j=1}^m  \Pr(\x_j \shortrightarrow \s_i).  
 \end{equation}   

Our next result shows that incentivizing creators to maximize user exposure can lead to significantly worse welfare.

\begin{proposition}\label{prop:unbound_user_welfare}
  Let $\tilde{\G}$ denote the variant of the \game{} $\G =(\{\S_i\}_{i=1}^n, \{\x_j\}_{j=1}^m, \sigma, \beta, K)$   by substituting player utility function in  \eqref{eq:player_utility_original} by the above \emph{user exposure} in \eqref{eq:player_utility_new}.  Then for any $K\geq 1, 0\leq\beta\leq \min\{0.14, \frac{1}{5\log K} \}$, there exist $\G$ and $\tilde{\G}$ such that 
    \begin{equation}\label{eq:poa_geq2}
        PoA(\tilde{\G})>2> PoA(\G).
    \end{equation}
     Moreover, when $K=1$ or $\beta$ approaches $0$, PoA$(\tilde{\G})$ can be arbitrarily large.
\end{proposition}

In stark contrast to Theorem \ref{thm:PoA} guaranteeing PoA$(\G)< 2$, Proposition \ref{prop:unbound_user_welfare} implies the deterioration of user welfare when content creators are incentivized to compete for the expected exposure of their content.  However, we find in practice both metrics are used: for example, user engagement has been used more often as a reward metric for established creators, whereas user exposure is used more for new creators \cite{meta_experiment,savy2019}. Our result serves as a theoretical defense for rewarding creators by user engagement if the system aims to improve overall welfare of the recommendations. 

To prove Proposition \ref{prop:unbound_user_welfare}, we construct a game instance in which the user welfare at NE is arbitrarily close to zero. 
Our construction also reveals interesting insights about situations where user welfare can be very bad. Hence, we briefly explain our construction here and leave our formal arguments in Appendix \ref{app:unbound_user_welfare}. 
Our constructed game has two groups of users: one \emph{dispersed} group that is fine with any content but is never very happy with it (i.e., a low relevant score for all content) and one \emph{focused} group who looks for a specific type of high-quality content (a high relevance score on such content); but only a small group of specialized creators can produce such high-quality content. However, if players are incentivized to compete for exposure, %their utilities are primarily determined by relative ranking rather than relevance scores. As a result, 
even creators from the small group tend to produce low-quality content that appeals to the dispersed group rather than high-quality content that benefits the focused group. This, in the worse case, can lead to arbitrarily worse welfare for the platform. 

%We remark that in practice, players' utility function can be cultivated by the system. That is, what metric the RS uses to reward creators -- e.g., user engagement or user exposure or any other metrics -- will naturally become the objective for the creators to optimize. In today's recommendation systems, both metrics have been used. To our knowledge, however,   On the research side,  recent works  \cite{ben2018competing,hron2022modeling} have also considered multi-agent RS with user exposure as the utility metric for creators. 

  
\vspace{2mm}
\noindent
\textbf{The welfare efficiency of top-$K$ recommendation policy.  } 
One may wonder whether the top-$K$ recommendation is indeed a good policy for securing the platform's welfare, i.e., is it possible that other recommendation policies (e.g., a probabilistic policy based on Plackett-Luce model \citep{plackett1975analysis,luce1959individual}) may even lead to better equilibrium outcomes? 
Our following analysis, as a corollary of Theorem \ref{thm:PoA}, shows that the answer is to some extent \emph{no} since \emph{any} recommendation policy cannot be better than the top-$K$ rule by more than a tiny fraction of the theoretical optimality. We believe this finding also serves as a theoretical justification for the wide adoption of the top-$K$ principle in practice. 

  % It would be desirable to extend the welfare guarantee to include matching mechanisms other than top-$K$, as it could be impractical to implement top-$K$ selection precisely due to various reasons. For example, the platform usually only has access to a noisy version of $\sigma$ since it needs to learn from data. Another reason is that the platform might want to deploy some probabilistic ranking models to increase exploration. Fortunately, Theorem \ref{thm:PoA} also demonstrates the inherent robustness of the top-$K$ recommendation principle, as deviations from generating the top-$K$ list result in a welfare loss fraction of at most $O(\frac{1}{\log K})$ relative to the optimal welfare. We formalize this claim in the following corollary of Theorem \ref{thm:PoA}.


\begin{corollary}\label{prop:welfare_loss}
Consider an arbitrary recommendation policy providing at most $K$ recommendations, which induces a different \game{} $\G'$. Let CCE$(\G')$ denote the corresponding CCE set of $\G'$ and $W(\G')=\min_{\al\in CCE(\G')}\EE_{\s\sim \al}[W(\s)]$ be its worst-case CCE welfare. Then we have  
    \begin{equation}\label{eq:welfare_loss_fraction}
        W(\G') \leq W(\G) + W^*_K / \Big(1+\frac{K\log (K+b)}{K+b}\Big),
    \end{equation}
    where $W^*_K$ is the best possible social welfare achieved via any centralized recommendation policy with $K$ slots.   

    %    Let $V_K=\min_{\al\in CCE(\G)}\EE_{\s\sim \al}[V(\s)]$ be the worst case social welfare when the system uses the top-$K$ matching principle, and $V'=\min_{\al\in CCE(\G')}\EE_{\s\sim \al}[V(\s)]$ be the corresponding value when the system switches to any other matching algorithm to generate matching result of length $K$. Then 
    % \begin{equation}\label{eq:welfare_loss_fraction}
    %     V'-V_K \leq V^*_K / \Big(1+\frac{K\log (K+b)}{K+b}\Big),
    % \end{equation}
    % where $V^*_K$ is the best possible social welfare over all possible strategy outcomes and system's matching algorithms.  
\end{corollary}

As indicated by \eqref{eq:welfare_loss_fraction}, the fraction of the loss of welfare is approximately $O(\frac{1}{\log K})$ as $\frac{K}{K+b}\sim O(1)$ when $K$ is large. The proof is straightforward based on Theorem \ref{thm:PoA} and can be found in Appendix \ref{app:welfare_loss}.

\subsection{Proof Highlights of Theorem \ref{thm:PoA}}\label{subsec:proof-sketch}

Our first step is to derive clean characterizations for the game primitives by utilizing properties of Gumbel distribution. The form of the user utility $\pi_j$ and welfare $W$ are corollaries of RU models \citep{baltas2001random}, however, the closed-form of the creator utility $u_i$ is a new property we derive. The results are summarized in the following Lemma \ref{lm:closed_form_utility}, and the detailed proof is deferred to Appendix \ref{app:close_utility}. 

\begin{lemma}\label{lm:closed_form_utility}
Given $\{ \varepsilon_i \}$ are drawn i.i.d.  from zero-mean Gumbel$(-\beta \gamma, \beta)$, the utility and welfare functions defined in \eqref{eq:user_utility_original}, \eqref{eq:player_utility_original} and \eqref{eq:welfare_original} have the following closed forms
\begin{equation}\label{eq:user_utility}
        \pi_j(\s)= \beta\log \Big[\sum_{\s_k\in\T_j(\s;K)} \exp{(\beta^{-1}\sigma(\s_k, \x_j))}\Big],
\end{equation}
\begin{equation}\label{eq:player_utility}
  u_i(\s)= \sum_{j=1}^m \pi_j(\s)\frac{\II[\s_i\in \T_j(\s;K)]\exp(\beta^{-1}\sigma(\s_i, \x_j))}{\sum_{\s_k\in \T_j(\s;K)} \exp(\beta^{-1}\sigma(\s_k, \x_j))},
\end{equation}
\begin{equation}\label{eq:welfare}
\!\!\!\!        W(\s)= \beta\sum_{j=1}^m \log \Big[\sum_{\s_k\in\T_j(\s;K)} \exp{(\beta^{-1}\sigma(\s_k, \x_j))}\Big].
\end{equation}
\end{lemma}

The main proof of Theorem \ref{thm:PoA} is based on a smoothness argument framework developed in the seminal work by \citet{roughgarden2015intrinsic}. For any strategy profile $\s$,  $W(\s) = \sum_i u_i(\s_i, \s_{-i}) $ is its  total  welfare function. A game is   $(\lambda,\mu)$\emph{-smooth} if  $ \lambda W(\s') - \mu W(\s) \leq \sum_i u_i(\s'_i, \s_{-i}) $ for any $(\s, \s') \in \S$. \citet{roughgarden2015intrinsic} observes that the PoA of any $(\lambda,\mu)$-smooth game  can be upper bounded by $\frac{1 + \mu}{\lambda}$. After plugging in the expression of $W(\s)$, the $(\lambda,\mu)$-smoothness condition can be re-written as
$$ 
    \sum_i [ \lambda u_i(\s'_i, \s'_{-i}) - u_i(\s'_i, \s_{-i})  ] \leq \sum_i  \mu u_i(\s) . 
$$
Intuitively, the smoothness parameters bound how much \emph{externality} other players' actions  (i.e., $\s'_{-i}$ or $\s_{-i}$) impose on any player $i$'s utility. Moreover, the tighter this bound is, the smoother the game is and the smaller the PoA is. To gain some intuition and also as a sanity check, consider the extreme situation in which each player's utility is not affected by other players' actions at all (i.e., the \emph{no externality} situation), we have $\lambda = 1$ and $\mu = 0$ implying PoA=1. That is, if any player's utility is not affected by others, then self-interested utility-maximizing behaviors also maximize social welfare, which is a straightforward observation. Certainly, we cannot hope for such a nice property to hold in general, but fortunately, many well-known games have been shown to be smooth. For example, second-price auctions are   $(1,1)$-smooth as shown by \citet{christodoulou2008bayesian},   congestion games are $(\frac{5}{3},\frac{1}{3})$-smooth as shown by \citet{roughgarden2015intrinsic}, and all-pay auctions are $(1/2,1)$-smooth as shown by \citet{roughgarden2017price}. 

Hence, the key challenge in proving Theorem \ref{thm:PoA} is to pin down the tightest possible $(\lambda, \mu)$ parameters for our \game{}. This boils down to a fundamental question in top-$K$ RS -- i.e., \emph{to what extent does the existence of other competing content creators affect a creator's utility}? To answer this question, we discover multiple interesting properties of the welfare and creator utility functions formulated as follows. Besides proving our main result in Theorem \ref{thm:PoA}, we believe these properties are also of interest for us to understand recommender systems. 
% \hf{Would it make sense to move the following lemma as part of the proof of Theorem 1? Again, you do not want your reader to read many technical lemmas before understanding your theorem, and you can absorb all the technicalities into your proof so long as they do not affect the reader's understanding about the messages/insights of your theorem. }\fan{I think maybe we can still have Lemma 1 here as it is part of the formulation of our game. We can put the discussion of it into the appendix as it is only introduced to simplify the technical analysis. }

Our second Lemma \ref{lm:submodular_V_} demonstrates the \emph{submodularity} of $W(\s)$. That is, the marginal gain of welfare from adding a new player decreases as the total number of creators increases. Lemma \ref{lm:utility_property_} further relates this marginal welfare increase with the added player's own utility. It shows that the increased welfare after introducing a new player $i$ with strategy $\s_i$ is at most   $i$'s utility  under  $\s_i$, multiplied by a shrinkage factor $c^{-1}(\beta, K) \in (0, 1]$. These two lemmas together allow us to prove that the \game{} is $(c^{-1}(\beta, K), c^{-1}(\beta, K))$-smooth, yielding Theorem \ref{thm:PoA}. Detailed proofs are presented in Appendix \ref{app:lemma23_proof}. % The detailed proof is provided in Appendix \ref{app:poa_proof} due to the closed form of the utility and welfare functions, which allows for a thorough analysis.

\begin{lemma}\label{lm:submodular_V_}[Submodularity of Welfare]
For any $\s=(\s_1,\cdots,\s_n)\in\S$, let $S=\{\s_1,\cdots,\s_n\}$. Then the social welfare function defined in Eq \eqref{eq:welfare_original} is submodular as a set function, i.e., for any $S, \s_x, \s_y$ it holds that
\begin{equation*}
    W(S\cup \{\s_x\})-W(S) \geq W(S\cup \{\s_x,\s_y\})-W(S\cup \{\s_y\}).
\end{equation*}
\end{lemma}

\begin{lemma}\label{lm:utility_property_} [Smoothness of Welfare]
For any $\s=(\s_1,\cdots,\s_n)\in\S$, $i\in[n]$ and $c(\beta, K)$ defined in Eq \eqref{eq:cbetaK_def}, player-$i$'s utility function $u_i(\s)$ defined in Eq \eqref{eq:player_utility_original} satisfies
\begin{equation*}
    W(\s)-W(\s_{-i}) \leq c^{-1}(\beta, K)\cdot u_i(\s_i;\s_{-i}).
\end{equation*}
\end{lemma}




% \section{Convergence Result with Continuous Action Space}

% \fan{We need to change the strategy about the presentation of this section. The motivation is we want to characterize when the concentration of strategies takes place. }

% In this section we establish 

% \subsection{Negative Result: \gamecap s with Cyclic Improvement Paths}


%         We have shown that if the user distribution and scoring function $\sigma$ satisfy condition \eqref{eq:suff_monotone}, DA dynamics always converge to the unique PNE of the game. Now we show a negative result which indicates that players' strategy sequence does not converge in general if the smoothness condition of $\sigma$ is violated . First we introduce two useful concepts:
        
%         \begin{definition}
%         In an $n-$player strategic game $\G(S_1,\dots,S_n,u_1,\dots,u_n)$, a profitable deviation is a join strategy pair $(\s,\s')\in \prod_{i=1}^n S_i\times \prod_{i=1}^n S_i$ such that $\s'=(s'_i,\s_{-i})$ for some $i$ and $u_i(\s')>u_i(\s)$. An improvement path is a maximal
%         sequence of profitable deviations.
%         \end{definition}
        
%         \begin{definition}
%         In an $n-$player strategic game $\G(S_1,\dots,S_n,u_1,\dots,u_n)$, a function $P:\prod_{i=1}^n S_i \rightarrow \RR$ is called a generalized ordinal potential of $\G$ if for any $i\in[n], \s_{-i}\in S_{-i}, s_i,s'_i\in S_i$, 
%         $$u_i(s_i,\s_{-i})>u_i(s'_i,\s_{-i}) \Longrightarrow P(s_i,\s_{-i})>P(s'_i,\s_{-i}).$$
%         \end{definition}
        
%         It is known that there is no cyclic improvement path in a generalized ordinal potential game, and any finite game with only finite improvement paths must possess a generalized ordinal potential:
%         \begin{proposition}\cite{monderer1996potential}
%         Every finite game $\G$ has a generalized ordinal potential
%         if and only if every improvement path of $\G$ is finite.
%         \end{proposition}
        
%         \begin{proposition}
%         When $n=2, \X=[0,1], \sigma(s_i,x)=5[1-(s_i-x)^2]$, $\G$ has a cyclic improvement path 
%         $$(0, \frac{2}{3})\rightarrow(0, \frac{1}{3})\rightarrow(1, \frac{1}{3})\rightarrow(1, \frac{2}{3})\rightarrow(0, \frac{2}{3}).$$
%         \end{proposition}
        
%         This example explicitly constructs a cyclic improvement path in a simple one-dimensional case and thus show the game does not have a potential structure in general. 


% \subsection{\gamecap ~as a Monotone Game}

% Next we demonstrate another interesting property of \game s. With a slight abuse of notation, we use $\frac{\partial \sigma}{\partial \s_i}$ to denote $\frac{\partial \sigma(\s;\x)}{\partial \s}|_{\s=\s_i}$, and use $\frac{\partial^2 \sigma}{\partial \s_i^2}$ to denote $\frac{\partial^2 \sigma(\s;\x)}{\partial \s^2}|_{\s=\s_i}$. We use $P\succ(\prec) 0$ to denote the matrix $P$ is positive (negative) definite. The next Theorem \ref{thm:monotone_game5} gives a sufficient condition such that $\G$ is a monotone game and thus enjoys several nice convergence properties.

% \begin{theorem}\label{thm:monotone_game5}
%    Suppose an \game ~$\G(\{\S_i\}_{i=1}^n, \X, \sigma, \beta, n)$ with continuous action space satisfies the following properties:
%    \begin{enumerate}
%        \item The scoring function $\sigma(\s,\x):\RR^d\times\RR^d\rightarrow \RR_{\geq 0}$ is twice differentiable w.r.t. $\s$,
%        \item $(\sigma, \X)$ satisfies that for any $\s=(\s_1,\cdots,\s_n)\in \S\subseteq \RR^{dn}$ and $i\in[n]$,
%    \begin{equation}\label{eq:suff_monotone}
%       \sum_{\x\in\X} \omega_i(\s,\x)\Big[\frac{\partial^2 \sigma}{\partial \s_i^2}+\Big(\frac{\partial \sigma}{\partial \s_i}\Big)\Big(\frac{\partial \sigma}{\partial \s_i}\Big)^{\top}\Big] \prec 0,
%    \end{equation}
%    where 
%    \begin{equation}
%        \omega_i(\s,\x)=p_i^2+(p_i-p_i^2)\log M,
%    \end{equation}
%    and
%     \begin{equation}
%        M=\sum_{i=1}^n\exp(\sigma(\s_i,\x)),p_i=\exp(\sigma(\s_i,\x))/M.
%    \end{equation}
%    \end{enumerate}
   
%    Then $\G$ is a monotone game and thus has a unique PNE. Moreover, if each player adopts a Dual Averaging (DA) algorithm with a strongly convex regularizer and a proper learning rate sequence (see Theorem 4.1 in \cite{mertikopoulos2019learning}), the strategy sequences converge to the PNE of $\G$. 
% \end{theorem}

% Theorem \ref{thm:monotone_game5} derives a sufficient condition for the scoring function and the user distribution under which the resultant producer competition game $\G$ is monotone. As indicated by properties of monotone games, the uniqueness of PNE and the convergence of DA dynamics are guaranteed. We also note that the result in Theorem \ref{thm:monotone_game5} is general as we do not introduce additional assumptions on the dimensionality of the action space, the scoring function $\sigma$, or the user population $\X$. To better understand the condition in Eq \eqref{eq:suff_monotone}, we point out a stronger condition that does not depend on the user population as follows:
% \begin{equation}\label{eq:21}
%     \frac{\partial^2 \sigma}{\partial \s_i^2}+\Big(\frac{\partial \sigma}{\partial \s_i}\Big)\Big(\frac{\partial \sigma}{\partial \s_i}\Big)^{\top} \prec 0, \forall i \in [n].
% \end{equation}

% \fan{see if we can derive any PoA result under the smooth condition for $\sigma$.}

% Eq \eqref{eq:21} requires function $\sigma(\s, \x)$ to be strictly concave in $\s$ and to be ``smooth" enough in the sense that the first-order gradient w.r.t. $\s$ is not very large. In general these requirements might seem too strong when putting together. However, as we will show later in the simulation, the smoothness requirement for $\sigma$ is actually less strict if we consider the full condition in Eq \eqref{eq:suff_monotone} by taking into account the user distribution. 






